Spatial Mappings for Planning and Optimization of Cellular Networks

In cellular networks, users are grouped into different cells and served by different access points (base stations) that provide wireless access to services and applications. In general, the service demand is very heterogeneous, non-uniformly distributed, and dynamic. Consequently, radio access networks create very irregular topologies with more access points where service demand is concentrated. While this dynamism requires networks with the ability to adapt to time-varying conditions, the non-uniformity of the service demand makes the planning, analysis, and optimization difficult. In order to help with these tasks, a framework based on canonical domains and spatial mappings (e.g., conformal mapping) have recently been proposed. The idea is to carry out part of the planning in a canonical (perfectly symmetric) domain that is connected to the physical one (real-scenario) by means of a spatial transformation designed to map the access points consistently with the service demand. This paper continues the research in that direction by introducing additional tools and possibilities to that framework, namely the use of centroidal Voronoi algorithms and non-conformal composite mappings. Moreover, power optimization is also introduced to the framework. The results show the usability and effectiveness of the proposed method and its promising research perspectives.

==> Section_Intro.tex <==
\subsection{Context and motivation}\label{Sec:Intro:Context}

Radio access planning and optimization are fundamental tasks in cellular networks. Broadly speaking, planning refers to the tasks of determining the number, location, and configuration of access points to provide wireless access to users (and \textit{things})
to services and applications, with a certain targeted Quality of Service~(QoS). In particular, the problem of finding the number of access points is also referred to as \textsl{dimensioning}~\cite{7368887}, and this initial step aims at providing the required capacity for the service demand volume that is expected. However, in practice, both dimensioning and sites positioning are very difficult problems because the service demand is not uniformly distributed and it is quite diverse and dynamic. Nowadays, taking into account the continuous evolution of radio access technologies, and the new concepts and paradigms that are expected for the fifth generation~(5G) of cellular networks, the boundary between planning and optimization tasks becomes blurred. Indeed, according to the excellent work presented in~\cite{7368887}, planning and optimization are iterative tasks that go \textit{hand-in-hand}. In this line of thinking, the authors of~\cite{7462493} also pose the need for re-thinking planning. They emphasize the importance of distributing the service demand as evenly as possible among cells as a key criterion to achieve effective planning; a goal that in the opinion of the authors of~\cite{7462493} (and in our's) is a very valid way to enhance system performance. 

In our previous work~\cite{7399421}, also motivated by the aforementioned ideas, a novel framework for planning and optimization based on the use of \textsl{canonical domains} and spatial transformations was presented. Therein, planning is addressed by breaking the problem into two parts: dimensioning and sites positioning, as it is shown in Fig.~\ref{Fig:PROP_FRAMEWORK}. The central idea is to carry out the dimensioning in a dual/canonical domain in which the service demand is uniformly distributed. In this manner, a regular network topology ($\mathcal{T}_{\rm c}$) with the required number of access points is obtained (Step 2). Then, sites positioning is performed by mapping the regular network topology ($\mathcal{T}_{\rm c}$) from the canonical domain ($\mathcal{R}$) onto the physical domain ($\mathcal{A}$) by means of a spatial mapping $F^{-1}:\mathcal{R}\rightarrow\mathcal{A}$ that corresponds to the inverse of another (previously computed) mapping $F:\mathcal{A}\rightarrow\mathcal{R}$. The idea is that, if the mapping $F$ is designed (Step 1) such that it maps $\mathcal{A}$ onto $\mathcal{R}$ redistributing the service demand uniformly, then $F^{-1}$ will map (Step 3) the access points from $\mathcal{R}$ onto $\mathcal{A}$ in a compatible manner with the service demand, i.e., the network topology $\mathcal{T}_{\rm p}$. In~\cite{7399421}, conformal mapping~\cite{papamichael2010numerical}, a mature field in Complex Analysis~\cite{ahlfors1953complex}, but previously unheard of in the context of cellular networks, was proposed to obtain the mappings $F$ and $F^{-1}$.
					\begin{figure}[t]
	    		\centering	    	
	    		\includegraphics[width = 0.90\textwidth]{FIGURES/PROP_FRAMEWORK1.pdf}
	    		\vspace{-0.65cm}\caption{Planning and optimization based on canonical domains and spatial mappings. The original problem introduced in~\cite{7399421} comprised Steps~1, 2, and 3 (direct and inverse mapping and analysis in the canonical domain). The proposed enhanced framework includes: generalizations for Step~1, alternative methods for Step~3, and integration of Step~4 (power optimization).}
	    		\label{Fig:PROP_FRAMEWORK}    		
			\end{figure}	
\subsection{Contribution}\label{Sec:Intro:Contrib}
The idea introduced in~\cite{7399421} is new and it represents a novel approach to network planning and optimization. However, as a technique in its infancy, it admits (and requires) further improvements and evolutions. Hence, we continue the work on this research problem by enriching the possibilities of the original framework (specifically  Steps~1~and~3, Fig.~\ref{Fig:PROP_FRAMEWORK}), and by integrating new tools~(Step~4). To be precise, the contributions of this paper can be summarized as follows: 
\begin{itemize}[leftmargin=0.75cm]
	\renewcommand{\labelitemi}{$\checkmark$} 
	\item The direct mapping (Step~1 in Fig.~\ref{Fig:PROP_FRAMEWORK}) is generalized using function composition~\cite{shapiro2012composition} to overcome the limitations of the mapping proposed in~\cite{7399421}. Thus, the new direct mapping includes both conformal and non-conformal transformations, and allows defining arbitrary spatial service demand distributions in the physical domain. 
	\item A new method for computing the inverse mapping~(Step~3 in Fig.~\ref{Fig:PROP_FRAMEWORK}) using the centroidal Voronoi algorithms~\cite{du1999centroidal} and power Voronoi diagrams~\cite{Tan2011} is presented and explained in this context. As it will be explained later on, this approach does not require the computation of the direct mapping $F$. 
	A comparative analysis between this technique and spatial mappings is also provided.
	\item Power optimization~(Step~4 in Fig.~\ref{Fig:PROP_FRAMEWORK}) to adjust the configuration of the network topologies in the physical domain is integrated into the framework. To the best of our knowledge, the proposed optimization formulation, although based on the existing load-coupling model~\cite{7340975}, is novel and has some convenient features from the planning point~of~view.
\end{itemize}
%The examples presented herein illustrate the use of the proposed enhancements, and the results clearly show their effectiveness of the proposed enhancements, and the effectiveness of the new tools now available for it. Examples and use cases have been selected to avoid any overlapping with the material previously presented~\cite{7399421}, but in such a way that the focus is placed on the novelties, and that they can be presented in a comprehensive manner. 
 
The rest of the paper is organized as follows: the next section provides a high level description of the enhanced framework. Generalizations and novelties for the spatial mappings are presented in Sections~\ref{Sec:DirectMapping}~and~\ref{Sec:InverseMapping}. The analysis in the canonical domain is, for the sake of completeness, briefly described in Section~\ref{Sec:AnalysisInCanDom}; it can be done following the methodology presented in~\mbox{\cite[\textsection$\,$IV]{7399421}.} The proposed power optimization is described in Section~\ref{Sec:PO}. Numerical examples are presented in Section~\ref{Sec:NR}. Section~\ref{Sec:Conclusions} closes the paper with conclusions and future research directions.













